An In-depth Look at Gemini's Language Abilities

The recently released Google Gemini class of models are the first to comprehensively report results that rival the OpenAI GPT series across a wide variety of tasks. In this paper, we do an in-depth exploration of Gemini's language abilities, making two contributions. First, we provide a third-party, objective comparison of the abilities of the OpenAI GPT and Google Gemini models with reproducible code and fully transparent results. Second, we take a closer look at the results, identifying areas where one of the two model classes excels. We perform this analysis over 10 datasets testing a variety of language abilities, including reasoning, answering knowledge-based questions, solving math problems, translating between languages, generating code, and acting as instruction-following agents. From this analysis, we find that Gemini Pro achieves accuracy that is close but slightly inferior to the corresponding GPT 3.5 Turbo on all tasks that we benchmarked. We further provide explanations for some of this under-performance, including failures in mathematical reasoning with many digits, sensitivity to multiple-choice answer ordering, aggressive content filtering, and others. We also identify areas where Gemini demonstrates comparably high performance, including generation into non-English languages, and handling longer and more complex reasoning chains. Code and data for reproduction can be found at https://github.com/neulab/gemini-benchmark

==> charts/bbh_compare_models.tex <==
\begin{figure}
\begin{subfigure}[t]{0.49\textwidth}
\includegraphics[trim=0 80 0 0, clip, width=\textwidth]{figures/reasoning-overall-accuracy-bbh.pdf}
\caption{Overall Accuracy}\label{fig:reasoning_overall_accuracy}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
~
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[trim=0 20 0 0, clip, width=\textwidth]{figures/reasoning-by-length-bbh.pdf}
    \caption{Accuracy by question length} \label{fig:reasoning_by_length}
\end{subfigure}
\caption{Accuracy on BIG-Bench-Hard}
\end{figure}


==> tables/code_case_study.tex <==

\newsavebox{\codeA}
\begin{lrbox}{\codeA}
\begin{minted}{python}
def f_3283984():
    """decode a hex string '4a4b4c' to UTF-8."""
\end{minted}
\end{lrbox}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{% 
\begin{tabular}{p{6cm}p{6cm}p{6cm}}
\toprule
\textbf{Input} & \textbf{Gemini Pro} & \textbf{GPT 3.5 Turbo} \\
\midrule
\usebox{\codeA}
% \begin{minipage}[t]{6cm}
% def f\_3283984():\\
% \hspace*{1em}"""decode a hex string '4a4b4c' to UTF-8."""
% \end{minipage}
&
\begin{minipage}[t]{6cm}
bytes(bytearray.fromhex('4a4b4c'), 'utf-8')
\end{minipage}
& 
\begin{minipage}[t]{6cm}
    hex\_string = '4a4b4c' \\
    decoded\_string =\\ bytes.fromhex(hex\_string).decode('utf-8') \\
    return decoded\_string
\end{minipage}
\\
\midrule
\begin{minipage}[t]{6cm}
from typing import List\\


def remove\_duplicates(numbers: List[int]) -> List[int]:\\
\hspace*{1em}""" From a list of integers, remove all elements that occur more than once.
    Keep order of elements left the same as in the input.
    >>> remove\_duplicates([1, 2, 3, 2, 4])
    [1, 3, 4]
    """
\end{minipage}& \begin{minipage}[t]{6cm}
    seen\_numbers = set()\\
    unique\_numbers = []\\
    for number in numbers:\\
    \hspace*{1em}    if number not in seen\_numbers:\\ \hspace*{2em}
            unique\_numbers.append(number)\\ \hspace*{2em}
            seen\_numbers.add(number)\\
    return unique\_numbers
\end{minipage} & \begin{minipage}[t]{6cm} return [x for x in numbers if numbers.count(x) == 1]
\end{minipage}
\\
\bottomrule
\end{tabular}}
\captionsetup{skip=10pt} % Adjust the space between the table and the caption
\caption{Case study of the code generation task where Gemini Pro fails but GPT 3.5 succeeds.}
\label{tab:code_case_study}
\end{table}
